SpicyMKL

We propose a new optimization algorithm for Multiple Kernel Learning (MKL) called SpicyMKL, which is applicable to general convex loss functions and general types of regularization. The proposed SpicyMKL iteratively solves smooth minimization problems. Thus, there is no need of solving SVM, LP, or QP internally. SpicyMKL can be viewed as a proximal minimization method and converges super-linearly. The cost of inner minimization is roughly proportional to the number of active kernels. Therefore, when we aim for a sparse kernel combination, our algorithm scales well against increasing number of kernels. Moreover, we give a general block-norm formulation of MKL that includes non-sparse regularizations, such as elastic-net and \ellp -norm regularizations. Extending SpicyMKL, we propose an efficient optimization method for the general regularization framework. Experimental results show that our algorithm is faster than existing methods especially when the number of kernels is large (> 1000).

==> mathdef.tex <==
%\newtheorem{defi}{Definition}
%\newtheorem{prop}[defi]{Proposition}
%\newtheorem{lemm}[defi]{Lemma}
%\newtheorem{theo}[defi]{Theorem}
%\newtheorem{coro}[defi]{Corollary}
%\newtheorem{exam}[defi]{Example}
%\newtheorem{fact}[defi]{Fact}
%\newtheorem{algo}[defi]{Algorithm}
%\newtheorem{claim}[defi]{Claim}
\newcommand{\theoproof}[1]{\noindent{\bf (Proof of Theorem #1) }}
\newcommand{\propproof}[1]{\noindent{\bf (Proof of Proposition #1) }}
\newcommand{\lemmproof}[1]{\noindent{\bf (Proof of Lemma #1) }\\}
\newcommand{\lemmproofn}[1]{\noindent{\bf (Proof of Lemma #1) }}
\newcommand{\coroproof}[1]{\noindent{\bf (Proof of Corollary #1) }\\}
%\newcommand{\proof}{\noindent\textbf{(Proof)} }
%\newcommand{\proofend}{\hfill$\Box$\vspace{2mm}}
%\newcommand{\QED}{\rule{7pt}{7pt}}

\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\define}{\stackrel{\mathrm{def}}{=}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\plim}{\mathop{\mathrm{plim}}}
\newcommand{\cov}[2]{\mathrm{Cov}(#1,#2)}
\newcommand{\rank}[1]{\mathrm{rank}\left(#1\right)}
\newcommand{\tr}[1]{\mathrm{tr}(#1)}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\sinc}{\mathrm{sinc}\;}
\newcommand{\unorm}[1]{\|#1\|}
\newcommand{\unorms}[1]{\unorm{#1}^2}
\newcommand{\inner}[2]{\langle #1,#2\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55

\newcommand{\mathbbC}{\mathbb{C}}
\newcommand{\mathbbE}{\mathbb{E}}
\newcommand{\mathbbN}{\mathbb{N}}
\newcommand{\mathbbR}{\mathbb{R}}
\newcommand{\boldzero}{{\boldsymbol{0}}}
\newcommand{\boldone}{{\boldsymbol{1}}}

\newcommand{\boldA}{{\boldsymbol{A}}}
\newcommand{\boldB}{{\boldsymbol{B}}}
\newcommand{\boldC}{{\boldsymbol{C}}}
\newcommand{\boldD}{{\boldsymbol{D}}}
\newcommand{\boldE}{{\boldsymbol{E}}}
\newcommand{\boldF}{{\boldsymbol{F}}}
\newcommand{\boldG}{{\boldsymbol{G}}}
\newcommand{\boldH}{{\boldsymbol{H}}}
\newcommand{\boldI}{{\boldsymbol{I}}}
\newcommand{\boldJ}{{\boldsymbol{J}}}
\newcommand{\boldK}{{\boldsymbol{K}}}
\newcommand{\boldL}{{\boldsymbol{L}}}
\newcommand{\boldM}{{\boldsymbol{M}}}
\newcommand{\boldN}{{\boldsymbol{N}}}
\newcommand{\boldO}{{\boldsymbol{O}}}
\newcommand{\boldP}{{\boldsymbol{P}}}
\newcommand{\boldQ}{{\boldsymbol{Q}}}
\newcommand{\boldR}{{\boldsymbol{R}}}
\newcommand{\boldS}{{\boldsymbol{S}}}
\newcommand{\boldT}{{\boldsymbol{T}}}
\newcommand{\boldU}{{\boldsymbol{U}}}
\newcommand{\boldV}{{\boldsymbol{V}}}
\newcommand{\boldW}{{\boldsymbol{W}}}
\newcommand{\boldX}{{\boldsymbol{X}}}
\newcommand{\boldY}{{\boldsymbol{Y}}}
\newcommand{\boldZ}{{\boldsymbol{Z}}}

\newcommand{\bolda}{{\boldsymbol{a}}}
\newcommand{\boldb}{{\boldsymbol{b}}}
\newcommand{\boldc}{{\boldsymbol{c}}}
\newcommand{\boldd}{{\boldsymbol{d}}}
\newcommand{\bolde}{{\boldsymbol{e}}}
\newcommand{\boldf}{{\boldsymbol{f}}}
\newcommand{\boldg}{{\boldsymbol{g}}}
\newcommand{\boldh}{{\boldsymbol{h}}}
\newcommand{\boldi}{{\boldsymbol{i}}}
\newcommand{\boldj}{{\boldsymbol{j}}}
\newcommand{\boldk}{{\boldsymbol{k}}}
\newcommand{\boldl}{{\boldsymbol{l}}}
\newcommand{\boldm}{{\boldsymbol{m}}}
\newcommand{\boldn}{{\boldsymbol{n}}}
\newcommand{\boldo}{{\boldsymbol{o}}}
\newcommand{\boldp}{{\boldsymbol{p}}}
\newcommand{\boldq}{{\boldsymbol{q}}}
\newcommand{\boldr}{{\boldsymbol{r}}}
\newcommand{\bolds}{{\boldsymbol{s}}}
\newcommand{\boldt}{{\boldsymbol{t}}}
\newcommand{\boldu}{{\boldsymbol{u}}}
\newcommand{\boldv}{{\boldsymbol{v}}}
\newcommand{\boldw}{{\boldsymbol{w}}}
\newcommand{\boldx}{{\boldsymbol{x}}}
\newcommand{\boldy}{{\boldsymbol{y}}}
\newcommand{\boldz}{{\boldsymbol{z}}}

\newcommand{\boldalpha}{{\boldsymbol{\alpha}}}
\newcommand{\boldbeta}{{\boldsymbol{\beta}}}
\newcommand{\boldzeta}{{\boldsymbol{\zeta}}}
\newcommand{\boldgamma}{{\boldsymbol{\gamma}}}
\newcommand{\bolddelta}{{\boldsymbol{\delta}}}
\newcommand{\boldepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\boldphi}{{\boldsymbol{\phi}}}
\newcommand{\boldvarphi}{{\boldsymbol{\varphi}}}
\newcommand{\boldPhi}{{\boldsymbol{\Phi}}}
\newcommand{\boldxi}{{\boldsymbol{\xi}}}
\newcommand{\boldeta}{{\boldsymbol{\eta}}}
\newcommand{\boldmu}{{\boldsymbol{\mu}}}
\newcommand{\boldomega}{{\boldsymbol{\omega}}}
\newcommand{\boldtheta}{{\boldsymbol{\theta}}}
\newcommand{\boldTheta}{{\boldsymbol{\Theta}}}
\newcommand{\boldSigma}{{\boldsymbol{\Sigma}}}


\newcommand{\calA}{{\mathcal A}}
\newcommand{\calB}{{\mathcal B}}
\newcommand{\calD}{{\mathcal D}}
\newcommand{\calF}{{\mathcal F}}
\newcommand{\calG}{{\mathcal G}}
\newcommand{\calL}{{\mathcal L}}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calN}{{\mathcal N}}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calR}{{\mathcal R}}
\newcommand{\calS}{{\mathcal S}}
\newcommand{\calT}{{\mathcal T}}
\newcommand{\calU}{{\mathcal U}}
\newcommand{\calH}{{\mathcal H}}
\newcommand{\calX}{{\mathcal X}}
\newcommand{\calY}{{\mathcal Y}}
\newcommand{\calZ}{{\mathcal Z}}
\newcommand{\calo}{{\mathcal o}}

\newcommand{\boldalphao}{{\overline{\boldalpha}}}
\newcommand{\boldalphah}{{\widehat{\boldalpha}}}
\newcommand{\boldalphat}{{\widetilde{\boldalpha}}}
\newcommand{\boldalphad}{{\boldalpha}'}
\newcommand{\bolddeltah}{{\widehat{\bolddelta}}}
\newcommand{\bolddeltat}{{\widetilde{\bolddelta}}}
\newcommand{\boldthetah}{{\widehat{\boldtheta}}}
\newcommand{\boldthetat}{{\widetilde{\boldtheta}}}
\newcommand{\boldbetao}{{\overline{\boldbeta}}}
\newcommand{\boldbetah}{{\widehat{\boldbeta}}}
\newcommand{\boldbetat}{{\widetilde{\boldbeta}}}
\newcommand{\boldzetah}{{\widehat{\boldzeta}}}
\newcommand{\boldzetat}{{\widetilde{\boldzeta}}}
\newcommand{\boldgammah}{{\widehat{\boldgamma}}}
\newcommand{\boldgammat}{{\widetilde{\boldgamma}}}
\newcommand{\boldxih}{{\widehat{\boldxi}}}
\newcommand{\boldxihd}{{\widehat{\boldxi}'}}
\newcommand{\boldxit}{{\widetilde{\boldxi}}}
\newcommand{\boldwh}{{\widehat{\boldw}}}
\newcommand{\alphao}{{\overline{\alpha}}}
\newcommand{\alphah}{{\widehat{\alpha}}}
\newcommand{\alphat}{{\widetilde{\alpha}}}
\newcommand{\alphad}{{\alpha}'}
\newcommand{\alphadh}{{\alphah}'}
\newcommand{\betao}{{\overline{\beta}}}
\newcommand{\betat}{{\widetilde{\beta}}}
\newcommand{\deltah}{{\widehat{\delta}}}
\newcommand{\deltat}{{\widetilde{\delta}}}
\newcommand{\xih}{{\widehat{\xi}}}
\newcommand{\xihd}{{\widehat{\xi}'}}
\newcommand{\xit}{{\widetilde{\xi}}}
\newcommand{\thetah}{{\widehat{\theta}}}
\newcommand{\betah}{{\widehat{\beta}}}
\newcommand{\weight}{w}
\newcommand{\weighth}{{\widehat{\weight}}}
\newcommand{\weighto}{{\overline{\weight}}}
\newcommand{\weightt}{{\widetilde{\weight}}}
\newcommand{\weightd}{{\weight}'}
\newcommand{\weightdh}{{\weighth}'}
\newcommand{\mh}{{\widehat{m}}}
\newcommand{\vh}{{\widehat{v}}}
\newcommand{\Sh}{{\widehat{S}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


\newcommand{\training}{\mathrm{tr}}
\newcommand{\test}{\mathrm{te}}
\newcommand{\inputox}{x^{\training}}
\newcommand{\inputx}{\boldx^{\training}}
\newcommand{\inputot}{x^{\test}}
\newcommand{\inputt}{\boldx^{\test}}
\newcommand{\outputx}{y^{\training}}
\newcommand{\outputt}{y^{\test}}
\newcommand{\outputth}{\widehat{y}^{\test}}
\newcommand{\regparam}{\lambda}
\newcommand{\regparamSIC}{\gamma}
\newcommand{\numexams}{n_{\training}}
\newcommand{\numtests}{n_{\test}}
%\newcommand{\numparams}{p}
\newcommand{\numparams}{b}
\newcommand{\numparamss}{t}
\newcommand{\inputdim}{d}
\newcommand{\RKHStarget}{{\calH}}
\newcommand{\RKHStargetp}{{\RKHStarget^\prime}}
\newcommand{\RKHSsub}{{\calS}}
\newcommand{\designmatrix}{{\boldX}}
\newcommand{\designmatrixtilde}{\widetilde{\designmatrix}}
\newcommand{\identitymatrix}{{\boldI}}
\newcommand{\kernelmatrix}{{\boldK}}
\newcommand{\learningmatrix}{{\boldL}}
\newcommand{\kernel}[2]{K(#1,#2)}
\newcommand{\Ezeta}{\mathbb{E}_\zeta}
\newcommand{\Enoise}{\mathbb{E}_\boldepsilon}
\newcommand{\Bxnoise}{B_{\boldx,\boldepsilon}}
% \newcommand{\Ex}{\mathop{\mathbb{E}}_{\{\boldx_i\}_{i=1}^\numexams}}
%\newcommand{\Exy}{\mathbb{E}_{\{(\boldx_i,y_i)\}_{i=1}^\numexams}}
\newcommand{\Ex}{\mathbb{E}_{\{\boldx_i\}_{i=1}^\numexams}}
\newcommand{\Exj}{\mathbb{E}_{\boldx_j}}
\newcommand{\Exnj}{\mathbb{E}_{\{\boldx_i\}_{i\neq j}}}
\newcommand{\Ey}{\mathbb{E}_{\{y_i\}_{i=1}^\numexams}}
\newcommand{\Eyj}{\mathbb{E}_{y_j}}
\newcommand{\Eynj}{\mathbb{E}_{\{y_i\}_{i\neq j}}}
\newcommand{\Etu}{\mathbb{E}_{(\boldt,u)}}
\newcommand{\Et}{\mathbb{E}_{\boldt}}
\newcommand{\Eu}{\mathbb{E}_{u}}
\newcommand{\param}{\alpha}
\newcommand{\learningtarget}{f}
\newcommand{\learningtargetp}{g}
\newcommand{\learningtargeto}{r}
%\newcommand{\learningresult}{\hat{f}^{(\numexams)}}
\newcommand{\learningresult}{\widehat{f}}
\newcommand{\gh}{\widehat{g}}
%\newcommand{\learningresultT}{\widehat{f}_{\calT_\numexams}}
%\newcommand{\learningresultTj}{\widehat{f}_{\calT_{\numexams\backslash j}}}
\newcommand{\learningresultTj}{\widehat{f}_{\calT_{j}}}
\newcommand{\learningresultj}{\widehat{f}_j}
\newcommand{\learningresultu}{\learningresult_u}
\newcommand{\weightoperator}{W}
%\newcommand{\learningtargetP}{\learningtarget_{\weightoperator\RKHSsub}
\newcommand{\learningtargetP}{g}
\newcommand{\learningtargetPb}{\learningtargetP^\bot}
\newcommand{\learningtargetPh}{\hat{\learningtargetP}}
\newcommand{\learningtargetPhu}{\learningtargetPh_u}
\newcommand{\learningoperator}{L}
\newcommand{\learningoperatoru}{\learningoperator_u}
\newcommand{\samplingoperator}{X}
\newcommand{\samplingoperatortrans}{\samplingoperator_{t}}
\newcommand{\inputdomain}{\calD}
\newcommand{\CL}{\mathrm{C}_\mathrm{L}}
%\newcommand{\SICPOI}{\mathrm{SIC}_\mathrm{POI}}
\newcommand{\XXX}{\mathrm{UTE}}
\newcommand{\YYY}{\mathrm{UWE}}
\newcommand{\SIC}{\mathrm{SIC}}
%\newcommand{\SIC}[1]{\mathrm{SIC}_{#1}}
% \newcommand{\ESE}[1]{\mathit{ESE}(#1)}
% \newcommand{\Bias}[1]{\mathit{Bias}(#1)}
% \newcommand{\Var}[1]{\mathit{Var}(#1)}
% \newcommand{\ESEhat}[1]{\widehat{\ESE{#1}}}
% \newcommand{\Biashat}[1]{\widehat{\Bias{#1}}}
% \newcommand{\Varhat}[1]{\widehat{\Var{#1}}}
\newcommand{\ESE}[1]{\mathit{ESE}_{#1}}
\newcommand{\Bias}[1]{\mathit{Bias}_{#1}}
\newcommand{\Var}[1]{\mathit{Var}_{#1}}
\newcommand{\ESEhat}[1]{\widehat{\mathit{ESE}}_{#1}}
\newcommand{\Biashat}[1]{\widehat{\mathit{Bias}}_{#1}}
\newcommand{\Biasshat}[1]{\widehat{\mathit{Bias}^2}_{#1}}
\newcommand{\Varhat}[1]{\widehat{\mathit{Var}}_{#1}}
\newcommand{\Keval}{d}
\newcommand{\Kevecy}{t}
\newcommand{\noisecovmatrix}{\boldQ}
\newcommand{\noisecovmatrixh}{\hat{\noisecovmatrix}}
\newcommand{\boldzt}{\boldz_{\learningtarget}}
\newcommand{\boldzp}{\boldz_{\learningtargetp}}
\newcommand{\boldzo}{\boldz_{\learningtargeto}}
\newcommand{\kernelmatrixv}{\kernelmatrix_{v}}
\newcommand{\boldHh}{\widehat{\boldH}}
\newcommand{\Hh}{\widehat{H}}
\newcommand{\Eh}{\widehat{E}}
\newcommand{\Dh}{\widehat{D}}
\newcommand{\boldhh}{\widehat{\boldh}}
\newcommand{\boldbh}{\widehat{\boldb}}
\newcommand{\boldah}{\widehat{\bolda}}
\newcommand{\hh}{\widehat{h}}
\newcommand{\boldht}{\widetilde{\boldh}}
\newcommand{\Ht}{\widetilde{H}}
\newcommand{\boldHt}{\widetilde{\boldH}}
\newcommand{\boldGh}{\widehat{\boldG}}
\newcommand{\boldEh}{\widehat{\boldE}}
\newcommand{\boldDh}{\widehat{\boldD}}
\newcommand{\boldAh}{\widehat{\boldA}}
\newcommand{\boldBh}{\widehat{\boldB}}
\newcommand{\boldCh}{\widehat{\boldC}}
\newcommand{\boldQh}{\widehat{\boldQ}}
\newcommand{\boldSh}{\widehat{\boldS}}
\newcommand{\boldTh}{\widehat{\boldT}}
\newcommand{\boldQt}{\widetilde{\boldQ}}
\newcommand{\boldWh}{\widehat{\boldW}}
% \newcommand{\boldWtilde}{\tilde{\boldW}}
\newcommand{\boldUh}{\widehat{\boldU}}
\newcommand{\boldUt}{\widetilde{\boldU}}
\newcommand{\calAo}{\overline{\calA}}
\newcommand{\calAh}{\widehat{\calA}}
\newcommand{\calBh}{\widehat{\calB}}
\newcommand{\calBt}{\widetilde{\calB}}
\newcommand{\learningmatrixWLSh}{\hat{\learningmatrix}_{w}}
\newcommand{\ph}{\widehat{p}}
\newcommand{\Pt}{P_{\test}}
\newcommand{\pt}{p_{\test}}
\newcommand{\pth}{\ph_{\test}}
\newcommand{\Px}{P_{\training}}
\newcommand{\px}{p_{\mathrm{x}}}
\newcommand{\pxh}{\ph_{\training}}
\newcommand{\yh}{\widehat{y}}
\newcommand{\RISKn}{R^{(\numexams)}}
\newcommand{\RISKnm}{R^{(\numexams-1)}}
% \newcommand{\RISKn}{R_\numexams}
% \newcommand{\RISKnm}{R_{\numexams-1}}
%\newcommand{\RISKnh}{\widehat{R}^{(\numexams)}}
%\newcommand{\RISKTh}{\widehat{R}_{\calT}}
\newcommand{\RISKhn}{\widehat{R}^{(\numexams)}}
\newcommand{\fold}{k}
%\newcommand{\loss}[3]{\ell\left(#1,#2,#3\right)}
\newcommand{\loss}[3]{\ell(#1,#2,#3)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\innerRKHS}[2]{\inner{#1}{#2}_\RKHStarget}
\newcommand{\unormRKHS}[1]{\unorm{#1}_\RKHStarget}
\newcommand{\unormRKHSs}[1]{\unormRKHS{#1}^2}
\newcommand{\trpRKHS}[1]{\trp{#1}_\RKHStarget}

\newcommand{\innerW}[2]{\inner{#1}{#2}_{\boldW}}
\newcommand{\unormW}[1]{\unorm{#1}_{\boldW}}
\newcommand{\unormWs}[1]{\unormW{#1}^2}

\newcommand{\samplingoperators}{\samplingoperator^\ast}
\newcommand{\samplingoperatord}{\samplingoperator^\dagger}

\newcommand{\numparamstilde}{\tilde{\numparams}}
\newcommand{\learningmatrixWLStilde}{\tilde{\learningmatrix}_{w}}

\newcommand{\learningmatrixt}{\learningmatrix^\top}
\newcommand{\learningmatrixs}{\learningmatrix^\ast}
\newcommand{\learningmatrixu}{\learningmatrix_u}
\newcommand{\learningmatrixuh}{\widehat{\learningmatrix}_u}
\newcommand{\learningmatrixut}{\widetilde{\learningmatrix}_u}
\newcommand{\learningmatrixWLS}{\learningmatrix_{w}}
%\newcommand{\learningmatrixutilde}{\widetilde{\learningmatrixu}}
\newcommand{\learningmatrixutilde}{\learningmatrix_r}
\newcommand{\learningmatrixutildet}{\learningmatrixutilde^\top}

\newcommand{\paramh}{\hat{\param}}
\newcommand{\paramt}{\tilde{\param}}
\newcommand{\paramast}{\param^\ast}
\newcommand{\vparam}{{\boldsymbol{\param}}}
\newcommand{\vparamast}{\vparam^\ast}
\newcommand{\vparamasttilde}{\tilde{\vparam}^\ast}
\newcommand{\vparamh}{\hat{\vparam}}
\newcommand{\vparamt}{\tilde{\vparam}}
\newcommand{\vparamhu}{\vparamh_u}
\newcommand{\vparamhr}{\vparamh_r}
\newcommand{\vparamhal}{\vparamh_{\param}}

\newcommand{\kernelmatrixi}{\kernelmatrix^{-1}}
\newcommand{\kernelmatrixd}{\kernelmatrix^{\dagger}}

\newcommand{\schatten}[2]{#1\otimes\overline{#2}}
\newcommand{\schattenp}[2]{\left(#1\otimes\overline{#2}\right)}
\newcommand{\schattennarrow}[2]{#1\!\otimes\!\overline{#2}}

\newcommand{\train}[1]{\left(x_{#1},y_{#1}\right)}
\newcommand{\trainh}{\left(\hat{x}_{m+1},\hat{y}_{m+1}\right)}
\newcommand{\trainhx}{ $\left(\hat{x}_{m+1}\right.$, $\left.\hat{y}_{m+1}\right)$ }
\newcommand{\repker}[1]{K\left(x,#1\right)}

\newcommand{\J}{J}
\newcommand{\Jh}{\widehat{\J}}
\newcommand{\preJh}{pre\Jh}
\newcommand{\Jw}{J_{w}}
\newcommand{\Jt}{J_{t}}
\newcommand{\JW}{J_{\boldW}}
\newcommand{\JH}{J_{\RKHStarget}}
\newcommand{\JT}{J_{T}}
\newcommand{\Bnoise}{B_\boldepsilon}
\newcommand{\Bzeta}{B_\zeta}
\newcommand{\C}{C}

\newcommand{\lambdah}{\widehat{\lambda}}

\newcommand{\sgmm}{\sigma_{m+1}}
\newcommand{\sgmmh}{\hat{\sigma}_{m+1}}
\newcommand{\sigmah}{\widehat{\sigma}}
\newcommand{\sgs}{\sigma^2}
\newcommand{\sgsu}{\sgs_u}
\newcommand{\sgsh}{\widehat{\sigma^2}}
\newcommand{\sgshu}{\widehat{\sigma^2_u}}
\newcommand{\sgst}{\tilde{\sigma}^2}
\newcommand{\sgq}{\sigma^4}

\newcommand{\smallninv}{{\textstyle\frac{1}{\numexams}}}
\newcommand{\iid}{\stackrel{i.i.d.}{\sim}}

% added by kana
% \newcommand{\Real}{\mathbb{R}}
% \def\tr{{\rm tr}}
% \def\te{{\rm te}}
% \def\ntr{{n_{\rm tr}}}
% \def\nte{{n_{\rm te}}}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End
